Minimizing Running Buffers for Tabletop Object Rearrangement: Complexity, Fast Algorithms, and Applications

For rearranging objects on tabletops with overhand grasps, temporarily relocating objects to some buffer space may be necessary. This raises the natural question of how many simultaneous storage spaces, or "running buffers", are required so that certain classes of tabletop rearrangement problems are feasible. In this work, we examine the problem for both labeled and unlabeled settings. On the structural side, we observe that finding the minimum number of running buffers (MRB) can be carried out on a dependency graph abstracted from a problem instance, and show that computing MRB is NP-hard. We then prove that under both labeled and unlabeled settings, even for uniform cylindrical objects, the number of required running buffers may grow unbounded as the number of objects to be rearranged increases. We further show that the bound for the unlabeled case is tight. On the algorithmic side, we develop effective exact algorithms for finding MRB for both labeled and unlabeled tabletop rearrangement problems, scalable to over a hundred objects under very high object density. More importantly, our algorithms also compute a sequence witnessing the computed MRB that can be used for solving object rearrangement tasks. Employing these algorithms, empirical evaluations reveal that random labeled and unlabeled instances, which more closely mimics real-world setups, generally have fairly small MRBs. Using real robot experiments, we demonstrate that the running buffer abstraction leads to state-of-the-art solutions for in-place rearrangement of many objects in tight, bounded workspace.

==> texs/00_paper-structure.tex <==

\begin{enumerate}
   \item introduction
   \item related works
   \item Preliminaries
   \begin{enumerate}
     \item formal definition of terms
     \item LRBM
     \item URBM
   \end{enumerate}
    \item Structural properties
    \begin{enumerate}
       \item Lower bound on URBM with discs
       \item Upper bound on URBM with discs
       \item Hardness of LRBM
     \end{enumerate}
     \item Algorithms
     \begin{enumerate}
         \item Dynamic Programming (able to adapt different requirements of the solution)
         \begin{enumerate}
             \item pseudo-codes
             \item working example
         \end{enumerate}
         \item DFDP (fast)
         \begin{enumerate}
             \item pseudo-codes
             \item working example
         \end{enumerate}
         \item ILP (able to adapt different requirements of the solution)
         \begin{enumerate}
             \item formulation
         \end{enumerate}
         \item priority queue based algorithm for URBM
         \begin{enumerate}
             \item reason to improve DP
         \end{enumerate}
     \end{enumerate}
     \item Application of RBM in TORI
     \begin{enumerate}
         \item introduction to TORI
         \item inherent and acquired constraints
         \item Lazy buffer allocation based on LRBM
            \begin{enumerate}
                \item computing primitive plans
                \begin{enumerate}
                    \item why RB matters in this case?\\
                    According to experiments, RBM can be solved faster than TBM while solution quality looks similar
                \end{enumerate}
                \item buffer allocation
                \begin{enumerate}
                    \item pseudo-codes
                    \item working example
                \end{enumerate}
                
            \end{enumerate}
        \item Bidirectional search with partial plans
        \item Preprocessing with URBM
        \begin{enumerate}
            \item working example
        \end{enumerate}
     \end{enumerate}
     \item Experiments
     \begin{enumerate}
         \item definition of density levels
         \item how do we generate instances (discs, cuboid)
         \item RBM experiments
         \begin{enumerate}
             \item LRBM
             \begin{enumerate}
                 \item algorithm performance on random cases
                 \item MRB on random instances
                 \item FVS vs MRB
             \end{enumerate}
             \item URBM
             \begin{enumerate}
                 \item algorithm performance on random cases
                 \item MRB on random instances
                 \item MRB on hard instances
             \end{enumerate}
         \end{enumerate}
         \item TORI experiments
         \begin{enumerate}
             \item primitive plans comparison (why RB rather than TB) RBM-SP-BST vs TBM-SP-BST vs RO-SP-BST
             \item with/without preprocessing comparison  (effectiveness of PP) RBM-SP-BST-PP vs RBM-SP-BST
             \item RBM-SP-BST comparing with other methods 
             \begin{enumerate}
                 \item three scenarios (large scale)
             \end{enumerate}
         \end{enumerate}
         \item Real robot demonstration
         \begin{enumerate}
             \item platform introduction
             \item external buffer setup with discs
             \begin{enumerate}
                 \item introducing environment
                 \item comparison between methods (RBM plan vs TBM plan)
             \end{enumerate}
             \item TORI
             \begin{enumerate}
                 \item introducing environment
                 \item comparison among methods(discs)
                 \item demo with cuboid object and objects with general shape: ``Rutgers Robotics'', ``Hello IJRR''
             \end{enumerate}
         \end{enumerate}
     \end{enumerate}
 \end{enumerate}
